Manifold Graph with Learned Prototypes for Semi-Supervised Image Classification

Recent advances in semi-supervised learning methods rely on estimating the categories of unlabeled data using a model trained on the labeled data (pseudo-labeling) and using the unlabeled data for various consistency-based regularization. In this work, we propose to explicitly leverage the structure of the data manifold based on a Manifold Graph constructed over the image instances within the feature space. Specifically, we propose an architecture based on graph networks that jointly optimizes feature extraction, graph connectivity, and feature propagation and aggregation to unlabeled data in an end-to-end manner. Further, we present a novel Prototype Generator for producing a diverse set of prototypes that compactly represent each category, which supports feature propagation. To evaluate our method, we first contribute a strong baseline that combines two consistency-based regularizers that already achieves state-of-the-art results especially with fewer labels. We then show that when combined with these regularizers, the proposed method facilitates the propagation of information from generated prototypes to image data to further improve results. We provide extensive qualitative and quantitative experimental results on semi-supervised benchmarks demonstrating the improvements arising from our design and show that our method achieves state-of-the-art performance when compared with existing methods using a single model and comparable with ensemble methods. Specifically, we achieve error rates of 3.35% on SVHN, 8.27% on CIFAR-10, and 33.83% on CIFAR-100. With much fewer labels, we surpass the state of the arts by significant margins of 41% relative error decrease on average.

==> sections/authors_long.tex <==
\author{%
  Chia-Wen Kuo\\
  Inst. for Robotics \& Intelligent Machines\\
  Georgia Institute of Technology\\
  Atlanta, GA 30332 \\
  \texttt{albert.cwkuo@gatech.edu} \\
  \And
  Chih-Yao Ma \\
  School of Electrical \& Computer Engineering \\
  Georgia Institute of Technology\\
  Atlanta, GA 30332 \\
  \texttt{cyma@gatech.edu} \\
  \AND
  Jia-Bin Huang \\
  Department of Electrical and Computer Engineering \\
  Virginia Polytechnic Institute and State University \\
  Blacksburg, VA 24061 \\
  \texttt{jbhuang@vt.edu} \\
  \And
  Zsolt Kira \\
  School of Interactive Computing \\
  Georgia Institute of Technology\\
  Atlanta, GA 30332 \\
  \texttt{zkira@gatech.edu} \\
}

==> tables/multihead.tex <==
\begin{table}[t]
\centering
\caption{Varying the number of graph network layers on the CIFAR-10 dataset (in error rate percentage).}
\label{table:multihead}
\begin{tabular}{r|c}
\toprule
Number of Layers                  &  Error \\
\hline \hline
1        &  ??? \\
2     & ??? \\
4        & ??? \\
8        & ??? \\
\bottomrule
\end{tabular}
\end{table}

==> tables/single-image.tex <==
\begin{table}[t]
\centering
\caption{
Proposed method with and without leveraging data in a mini-batch.
}
\label{table:single-image}
\small
\begin{tabular}{rccc}
\toprule
Method                  & CIFAR-10                  & CIFAR-100                 \\ 
\midrule
$\Pi$-VAT (baseline) & 9.20 $\pm$ 0.02    &  34.94 $\pm$ 0.24                  \\
Ours w/o mini-batch &  8.83 $\pm$ 0.14    & 34.24 $\pm$ 0.18\\
Ours w/ mini-batch &   8.76 $\pm$ 0.05             &  34.01 $\pm$ 0.12 \\
\bottomrule
\end{tabular}
\end{table}

